Shoulders of Giants: A Look at the Degree and Utility of Openness in NLP Research

We analysed a sample of NLP research papers archived in ACL Anthology as an attempt to quantify the degree of openness and the benefit of such an open culture in the NLP community. We observe that papers published in different NLP venues show different patterns related to artefact reuse. We also note that more than 30% of the papers we analysed do not release their artefacts publicly, despite promising to do so. Further, we observe a wide language-wise disparity in publicly available NLP-related artefacts.

==> tables/TaskDF_old.tex <==
Corpora & 19 & 22 & 11 & 11 & 11 & 74 \\
Translation & 10 & 12 & 8 & 6 & 10 & 46 \\
Morphological Analyzer & 11 & 8 & 2 & 3 & 1 & 25 \\
Automatic Speech Recognition (ASR) & 5 & 1 & 10 & 4 & 3 & 23 \\
Data Sets & 6 & 1 & 5 & 3 & 4 & 19 \\
Parsers & 4 & 5 & 3 & 1 & 3 & 16 \\
Language Model & 1 & 2 & 10 & 1 & 2 & 16 \\
Named-Entity Recognition (NER) & 1 & 0 & 3 & 5 & 7 & 16 \\
Dictionary/Lexicon & 6 & 4 & 1 & 1 & 3 & 15 \\
Cross-Lingual Applications & 2 & 1 & 3 & 6 & 2 & 14 \\
Part of Speech (PoS) & 1 & 6 & 3 & 2 & 2 & 14 \\
Hate Speech Detection & 0 & 0 & 2 & 6 & 1 & 9 \\
Misinformation Detection & 0 & 0 & 0 & 4 & 3 & 7 \\
Text Classification & 1 & 2 & 1 & 2 & 1 & 7 \\
Question and Answer (QnA) & 0 & 1 & 2 & 1 & 3 & 7 \\
Wordnets/Ontology/Taxonomy & 3 & 1 & 0 & 2 & 0 & 6 \\
Text Generation & 0 & 0 & 0 & 0 & 6 & 6 \\
NLP Tools & 1 & 4 & 1 & 0 & 0 & 6 \\
Discourse Analysis & 0 & 2 & 1 & 1 & 2 & 6 \\
Phonological Analyzer & 0 & 1 & 0 & 2 & 1 & 4 \\
Multiple Tasks & 0 & 0 & 1 & 3 & 0 & 4 \\
Semantic Similarity & 0 & 0 & 0 & 3 & 1 & 4 \\
Sentiment Analyzer & 0 & 0 & 1 & 1 & 2 & 4 \\
Summarizing & 0 & 0 & 0 & 3 & 1 & 4 \\
Spelling and Grammar & 0 & 1 & 1 & 0 & 1 & 3 \\
Coreference Resolution & 0 & 0 & 0 & 0 & 3 & 3 \\
Text-to-Speech & 0 & 2 & 1 & 0 & 0 & 3 \\
Tokenizer & 0 & 0 & 1 & 2 & 0 & 3 \\
Lexical Inference & 0 & 0 & 0 & 0 & 3 & 3 \\
Transliteration & 0 & 0 & 2 & 0 & 1 & 3 \\
Information Extraction & 0 & 0 & 1 & 1 & 0 & 2 \\
Bilingual Lexicon Induction (BLI) & 0 & 1 & 0 & 0 & 1 & 2 \\
Text Classification & 0 & 0 & 1 & 0 & 0 & 1 \\
Optical Character Recognition (OCR) & 0 & 1 & 0 & 0 & 0 & 1 \\
Intent Detection & 1 & 0 & 0 & 0 & 0 & 1 \\
News/Social Media Recommendation & 0 & 0 & 0 & 0 & 1 & 1 \\
Stemming & 0 & 0 & 0 & 0 & 1 & 1 \\
Semantic (Other) & 0 & 0 & 0 & 0 & 1 & 1 \\
Language Identification (LangID) & 0 & 0 & 1 & 0 & 0 & 1 \\
\hline
\textbf{Total} & 72 & 78 & 76 & 74 & 81 & 381 
